Transfer Faster, Price Smarter: Minimax Dynamic Pricing under Cross-Market Preference Shift

We study contextual dynamic pricing when a target market can leverage K auxiliary markets -- offline logs or concurrent streams -- whose mean utilities differ by a structured preference shift. We propose Cross-Market Transfer Dynamic Pricing (CM-TDP), the first algorithm that provably handles such model-shift transfer and delivers minimax-optimal regret for both linear and non-parametric utility models. For linear utilities of dimension d, where the difference between source- and target-task coefficients is $s_{0}$-sparse, CM-TDP attains regret $\tilde{O}((d*K^{-1}+s_{0})\log T)$. For nonlinear demand residing in a reproducing kernel Hilbert space with effective dimension $\alpha$, complexity $\beta$ and task-similarity parameter $H$, the regret becomes $\tilde{O}\!(K^{-2\alpha\beta/(2\alpha\beta+1)}T^{1/(2\alpha\beta+1)} + H^{2/(2\alpha+1)}T^{1/(2\alpha+1)})$, matching information-theoretic lower bounds up to logarithmic factors. The RKHS bound is the first of its kind for transfer pricing and is of independent interest. Extensive simulations show up to 50% lower cumulative regret and 5 times faster learning relative to single-market pricing baselines. By bridging transfer learning, robust aggregation, and revenue optimization, CM-TDP moves toward pricing systems that transfer faster, price smarter.

==> NeurIPS2025/0-intro-1.tex <==
\section{Introduction}\label{sec:intro}

Dynamic pricing systems have matured to the point where ride-sharing platforms,
online travel agencies, and retail marketplaces
update thousands of prices per minute.
Yet each \emph{new} city, product line, or
advertising campaign typically begins with only a handful of transactions,
forcing the algorithm to
re-learn demand parameters from a cold start.
This data scarcity slows revenue convergence
and accentuates early-stage price misalignment—precisely when managerial attention is highest.

A natural remedy is to \emph{transfer} knowledge from related markets:
a ski-rental shop in Aspen should inform one in Vail,
and a newly launched streaming plan should learn from existing tiers.
Transfer learning has delivered impressive gains in
vision and language models,
but the theory and practice of \emph{online revenue learning} are still dominated by
single-market methods~\citep{javanmard2019dynamic,tullii2024improved}.  Existing
meta-pricing work pools data only offline or under restrictive covariate shift
assumptions~\citep{bastani2022meta,wang2025transfer}, leaving open the central
question:

\begin{center}
\emph{How can an algorithm price competitively in a new market while
simultaneously harvesting and correcting information from several heterogeneous
source markets?}
\end{center}

\textbf{Our answer: Cross-Market Transfer Dynamic Pricing (CM-TDP).}
CM-TDP operates in two lightweight steps \emph{every} time new data arrive:

\vspace{-0.25em}
\begin{enumerate}[leftmargin=1.5em,topsep=2pt,itemsep=2pt]
\item \textbf{Bias-corrected aggregation.}  A ridge-type estimator 
pools $K$ auxiliary markets, then a sparse (or kernel) debiasing step
aligns it with fresh target data—yielding a plug-in demand model that is
continuously refined.
\item \textbf{Revenue-aware exploration.}  Prices are posted via an
optimistic plug-in rule, ensuring exploration–exploitation balance
\emph{without} handcrafted schedules or prior tuning.
\end{enumerate}
\vspace{-0.25em}

\paragraph{Why is this new?}
CM-TDP bridges three literatures that have so far evolved in parallel:
dynamic pricing, multitask contextual bandits, and online meta-learning.
It is \emph{(i)} the first pricing algorithm to accommodate \emph{utility-model shift} - the realistic scenario where mean utilities differ across markets—while leveraging \emph{multiple} sources,
\emph{(ii)} the first to provide minimax-type \emph{regret} guarantees for
\textbf{both} sparse-linear and RKHS-smooth utilities, and \emph{(iii)} a single
procedure that works in \emph{online-to-online} (all markets live) and
\emph{offline-to-online} (historical data only) settings.

\paragraph{Technical contributions.}
\begin{itemize}[leftmargin=1.5em,topsep=2pt,itemsep=2pt]
\item \textbf{Unified transfer framework.}  We formalise a
general notion of \emph{utility shift} and instantiate CM-TDP for
sparse-linear and RKHS demand classes (Secs.~\ref{sec:algo-thm}–\ref{sec:rkhs-extension}).
\item \textbf{Optimal regret bounds.} 
For dimension $d$, sparsity $s_0$ and
$K$ sources, CM-TDP achieves
\(
\tilde{\mathcal O}\!\bigl( (d/K + s_0)\log T \bigr)
\)
regret in the linear case, and
\(
\tilde{\mathcal O}\!\bigl( K^{-2\alpha\beta/(2\alpha\beta+1)}T^{1/(2\alpha\beta+1)}
      + H^{2/(2\alpha+1)}T^{1/(2\alpha+1)} \bigr)
\)
in the RKHS case—matching information-theoretic lower bounds up to
log factors (Thms.~\ref{thm:upper-single-homo-linear-o2o} and
\ref{thm:upper-single-homo-RKHS-o2o}).
\item \textbf{Scalable implementation \& evidence.}
Extensive simulations and real e-commerce traces show up to
\textbf{35\% more revenue} and \textbf{7× faster} convergence than the best
single-market and meta-pricing baselines (Sec.~\ref{sec:exps}).
\end{itemize}

\paragraph{Implications.}
By unifying transfer learning, contextual bandits, and pricing theory,
CM-TDP enables practitioners to bootstrap a pricing engine in one market
using data already collected elsewhere—\emph{exactly once}, not $K$ times.
The framework is lightweight enough for real-time deployment and general
enough to inspire follow-up work on robustness, product interactions,
and fairness in algorithmic pricing.

The remainder of the paper proceeds as follows:
Sec.~\ref{sec:prob-setting} formalises the random-utility transfer model,
Secs.~\ref{sec:algo-thm}–\ref{sec:rkhs-extension} present algorithms and
theoretical guarantees, Sec.~\ref{sec:exps} reports empirical results, and
Sec.~\ref{sec:conclusion} discusses future directions.

==> NeurIPS2025/3-proofs/34-prop-single-part2-tight.tex <==


Define the event $\mathcal{B}_n$ as follows:
\begin{equation*}
\mathcal{B}_n \equiv \left\{ X \in \mathbb{R}^{n_0 \times d} : \sigma_{\min}(X^\top X / n_0) > C_{\min} / 2 \right\}.
\end{equation*}

Using concentration bounds on the spectrum of random matrices with subgaussian rows (\cite{vershynin2011asymptoticanalysis}, Equation 5.26), there exist constants $c, c_1 > 0$ such that for $n > c_1 d$, we have $\mathbb{P}(\mathcal{B}_n) \geq 1 - e^{-c n_0^2}$.

For $\gamma > 0$, we define the event $\mathcal{F}_\gamma = \{ \|\nabla \mathcal{L}(\bbeta^{(ag)})\|_\infty \leq \gamma \}$. Using Equation~\ref{eqn:5-gradient-hessian}, and by applying Azuma-Hoeffding inequality, we obtain
\begin{equation}\label{eqn:13-define-f-tight}
\mathbb{P}(\mathcal{F}_\gamma) \geq 1 - d \exp \left( -\frac{n_0 \gamma^2}{2 u_F^2} \right).
\end{equation}

We also let $\mathcal{E}_{1,n} \equiv \mathcal{B}_n \cap \mathcal{F}_{\lambda/2}$, $\mathcal{E}_{2,n} \equiv \mathcal{B}_n \cap \mathcal{F}_{\lambda/2}^c$. To lighten the notation, we use the shorthand $D \equiv \|\bbeta^{(ag)} - \hat{\bbeta}^{(ag)}\|_2^2$.
We then have
\begin{equation*}
\mathbb{E}(D) = \mathbb{E}(D \cdot \mathbb{I}(\mathcal{B}_n^c)) + \mathbb{E}(D \cdot \mathbb{I}(\mathcal{E}_{1,n})) + \mathbb{E}(D \cdot \mathbb{I}(\mathcal{E}_{2,n})).
\end{equation*}

We treat each of the terms on the right-hand side separately.

\begin{itemize}
    \item \textbf{Term 1:} We have
    \begin{equation}\label{eqn:12-term1}
    \mathbb{E}(D \cdot \mathbb{I}(\mathcal{B}_n^c)) \leq 4W^2 \mathbb{P}(\mathcal{B}_n^c) \leq 4W^2 e^{-c n_0^2}.
    \end{equation}
    
    \item \textbf{Term 2:} Similar to proof of Proposition \ref{prop:upper-single-homo-linear-o2o-2}, on $\mathcal{E}_{1,n}$, we have $D \leq c_1s_0\log d/ n_0$. Hence,
    \begin{equation}\label{eqn:12-term2}
    \mathbb{E}(D \cdot \mathbb{I}(\mathcal{E}_{1,n})) \leq c_1\frac{s_0 \log d}{n_0}.
    \end{equation}
    
    \item \textbf{Term 3:} To bound term 3, we first prove the following lemma.
\end{itemize}

\begin{lemma}\label{lemma:upper-single-homo-linear-o2o-tight-item3}
    On event $\mathcal{E}_n(\gamma) \equiv \mathcal{B}_n \cap \mathcal{F}_\gamma$, with $\gamma > \lambda/2$, we have
\begin{equation*}
D \leq \left( \frac{36}{C_{\min}^2 \ell_F^2} \right) \gamma^2 d.
\end{equation*}
\end{lemma}

We next bound term 3 as follows. Let $L = 9\lambda^2 d / (C_{\min}^2 \ell_F^2)$.

\begin{align}\label{eqn:12-term3-0}
    \mathbb{E}(D \cdot \mathbb{I}(\mathcal{E}_{2,n})) &= \int_0^\infty \mathbb{P}(D \cdot \mathbb{I}(\mathcal{E}_{2,n}) > \alpha) \mathrm{d}\alpha= L \int_0^\infty \mathbb{P}(D \cdot \mathbb{I}(\mathcal{E}_{2,n}) > Lc) \mathrm{d}c\\
    & = L \int_0^1 \mathbb{P}(D \cdot \mathbb{I}(\mathcal{E}_{2,n}) > Lc) \mathrm{d}c + L \int_1^\infty \mathbb{P}(D \cdot \mathbb{I}(\mathcal{E}_{2,n}) > Lc) \mathrm{d}c.
\end{align}

For the first term on the \emph{r.h.s.} we write
\begin{equation}\label{eqn:12-term3-1}
L \int_0^1 \mathbb{P}(D \cdot \mathbb{I}(\mathcal{E}_{2,n}) > Lc) \mathrm{d}c \leq L \int_0^1 \mathbb{P}(\mathcal{E}_{2,n}) \leq L \mathbb{P}(\mathcal{F}_{\lambda/2}^c) \leq \frac{L}{d},
\end{equation}
where the last step holds from Equation~\ref{eqn:13-define-f-tight} with $\gamma = \lambda/2$.

We next upper bound the second term. For arbitrary fixed $c > 1$, let $\gamma = \sqrt{Lc / (d\kappa)}$, with $\kappa = 36 / (\ell_F^2 C_{\min}^2)$. It is easy to verify that $\gamma = \sqrt{c} \lambda / 2 > \lambda / 2$. Further, by Lemma \ref{lemma:upper-single-homo-linear-o2o-tight-item3}, on $\mathcal{E}(\gamma)$ we have $D \leq \kappa \gamma^2 d = Lc$. Hence,
\begin{equation}\label{eqn:14-2}
\mathbb{P}(D \cdot \mathbb{I}(\mathcal{E}_{2,n}) > Lc) \leq \mathbb{P}(\mathcal{E}(\gamma)^c \cap \mathcal{E}_{2,n}) \leq \mathbb{P}(\mathcal{F}_\gamma^c \cap \mathcal{B}_n) \leq \mathbb{P}(\mathcal{F}_\gamma^c).
\end{equation}

Further, applying Equation~\ref{eqn:13-define-f-tight} and plugging for $\gamma$, we obtain
\begin{equation}\label{eqn:14-1}
\mathbb{P}(\mathcal{F}_\gamma^c) \leq d \exp \left( -\frac{n L c}{2 u_F^2 \kappa d} \right) = d \exp \left( -\frac{n \lambda^2}{8 u_F^2} \right) \leq d^{1-2c}.
\end{equation}
Here, the second step follows from definition of $L$ and the last step holds because $\lambda \geq 4 u_F \sqrt{(\log d) / n_0}$.

Combining Equations~\ref{eqn:14-1} and~\ref{eqn:14-2}, we have
\begin{equation}\label{eqn:12-term3-2}
L \int_1^\infty \mathbb{P} \left( D \cdot \mathbb{I}(\mathcal{E}_{2,n}) > Lc \right) \mathrm{d}c \leq L \int_1^\infty d^{1-2c} \mathrm{d}c \leq \frac{L}{2 d \log d}.
\end{equation}

Using bounds~\ref{eqn:12-term3-1} and~\ref{eqn:12-term3-2} in Equation~\ref{eqn:12-term3-0}, we obtain
\begin{equation}
\mathbb{E}(D \cdot \mathbb{I}(\mathcal{E}_{2,n})) \leq \frac{L}{d} \left( 1 + \frac{1}{2 \log d} \right) \leq \frac{3L}{2d} < \frac{16 \lambda^2}{\ell_F^2 C_{\min}^2}=\frac{c_1'\log d}{n_0}.
\end{equation}

The result follows by putting the upper bounds on the three terms, cf. Equations~\ref{eqn:12-term1},  ~\ref{eqn:12-term2}, together.

==> NeurIPS2025/5-algo-complete.tex <==
\begin{algorithm}[!ht]
\caption{Offline-to-online Cross-market Pricing Transfer with Linear Utility Model} \label{algo:trans-pricing-single-f2o-ns}
\KwInput{Offline source market data $ \{ (p_t^{(k)}, \bx_t^{(k)}, y_t^{(k)}) \}_{t \in \calH^{(k)}} $ for $k \in [K]$; feature vector $ \{\bx_t^{(0)}\}_{t \in \mathbb{N}} $ for the target market} 

\tcc{******* Initial Warm-up *******}
Compute the initial estimate of coefficient using the source data
\begin{equation*}
    \hat\bbeta^{\rm (ag)} = \argmin_{\mathbf{b}} \, \Big\{ \frac{1}{n_\calK} \sum_{k \in [K]} \sum_{t \in \calH^{(k)}}
    L(\mathbf{b}; p_t^{(k)}  \bx_t^{(k)}, y_t^{(k)}) ) \Big\}
\end{equation*}

Apply the price  $\hat{p}_1^{(0)}  = h ( \bx_1^{(0)} \cdot \hat{\bbeta}^{\rm(ag)} )$  to $\bx_1^{(0)}$ and collect data $(\hat{p}_1^{(0)}, \bx_1^{(0)}, y_1^{(0)})$.

\tcc{******* Update Estimate with transfer learning *******}


\For{each $m = 2, \ldots, n_0 $} {
Set the length of the $m$-th episode: $\ell_m :=  2^{m - 1}$

Update the parameter $ \hat{\bbeta}_{m} $ using the observations in the $(m-1)$-th episode and the source markets: 

\begin{equation*}
    \hat{\bbeta}_{m}^{(0)} := \hat{\bbeta}^{\rm (ag)} + \hat{\bdelta}_{m}.
\end{equation*}

where
 \begin{equation*}
 \begin{split}
     \hat{\bdelta}_{m}  & := \argmin_{\bdelta} \, \Big\{ \frac{1}{\ell_{m-1}} \sum_{t = 2^{m-2} }^{2^{m-1} - 1} L(\hat{\bbeta}^{\rm(ag)}+\bdelta; \hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)}) + \lambda_m \| \bdelta \|_1  \Big\}.
\end{split}
 \end{equation*}

 For each time $ t \in [2^{m-1},  2^{m} - 1] $ in the $m$-th episode, apply price $\hat{p}_t^{(0)} := h(\bx_t^{(0)} \cdot \hat{\bbeta}_{m}^{(0)})$ and collect data $(\hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})$.
}

\tcc{******* Update Estimate without transfer learning *******}


\For{each $m \geq n_0 + 1$} {
Set the length of the $m$-th episode: $\ell_m :=  2^{m - 1}$

Update the parameter $ \hat{\bbeta}_{m}^{(0)} $ using only the observations in the $(m-1)$-th episode: 

 \begin{equation*}
 \begin{split}
     \hat{\bbeta}_{m}^{(0)}  & := \argmin_{\mathbf{b}} \, \Big\{ \frac{1}{\ell_{m-1}}  \sum_{t = 2^{m-2} }^{2^{m-1} - 1} L(\mathbf{b}; \hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})  \Big\}.
\end{split}
 \end{equation*}

 For each time $   t \in [2^{m-1},  2^{m} - 1] $ in the $m$-th episode, apply price $\hat{p}_t^{(0)} := h(\bx_t^{(0)} \cdot \hat{\bbeta}_{m}^{(0)})$ and collect data $(\hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})$.
}

\KwOutput{Offered price $\hat{p}_t^{(0)}$, $t \geq 1$}
\end{algorithm}


\begin{algorithm}[!ht]
\caption{Online-to-online Cross-Market Pricing Transfer with Linear Utility Model} \label{algo:trans-pricing-single-o2o-ns}
\KwInput{Online source market data $ \{ (\bp_t^{(k)}, \bX_t^{(k)}, \by_t^{(k)}) \}_{t \in \calH^{(k)}_m} $ for $k \in [K]$; feature matrix $ \{\bX_t^{(0)}\}_{t \in \mathbb{N}} $ for the target market} 


$l_1 \leftarrow 1, \, p_1^{(0)} \leftarrow 0, \, \hat{\beta}^{(0)}_0 \leftarrow 0$

\For{each $m = 2, 3,\ldots$} {
Set the length of the $m$-th episode: $\ell_m :=  2^{m - 1}$

\tcc{******* Initial Estimate Using Source Market Data *******}
Compute the initial estimate $\hat\bbeta^{\rm (ag)}_m$ using the source data in the $(m-1)$-th episode

\begin{equation*}
\hat\bbeta^{\rm (ag)}_m = \argmin_{\mathbf{b}} \, \Big\{ \frac{1}{K l_{m-1}} \sum_{k \in [K]} \sum_{t \in \calH^{(k)}_{m-1}}
L(\mathbf{b}; p_t^{(k)}  \bx_t^{(k)}, y_t^{(k)}) ) \Big\}
\end{equation*}
where the function 
\begin{equation}\label{eqn:0-MLE}
\begin{split}
L(\mathbf{b}; p,  \bx, y ) ) & := -   \Big\{ \mathbbm{1} (y  = 1) \log (1 - F(p - \mathbf{b} \cdot \bx   ))  +  \mathbbm{1} (y  = 0) \log ( F(p  - \mathbf{b} \cdot \bx    )) \Big\}.
\end{split}
\end{equation}

\tcc{******* Update Estimate Using Target Market Data *******}
Update the parameter $ \hat{\bbeta}_{m}^{(0)} $ using the observations in the $(m-1)$-th episode and the source markets: 

\begin{equation*}
\hat{\bbeta}_{m}^{(0)} := \hat{\bbeta}^{\rm (ag)}_m + \hat{\bdelta}_{m}
\end{equation*}

where
\begin{equation*}
\begin{split}
\hat{\bdelta}_{m}  & := \argmin_{\bdelta} \, \Big\{ \frac{1}{\ell_{m-1}} \sum_{t = 2^{m-2} }^{2^{m-1} - 1} L(\hat{\bbeta}^{\rm(ag)}_m+\bdelta; \hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)}) + \lambda_m \| \bdelta \|_1  \Big\}.
\end{split}
\end{equation*}

\tcc{******* Pricing Decision *******}
For each period $ t \in [2^{m-1},  2^{m} - 1] $ in the $m$-th episode, apply price $\hat{p}_t^{(0)} := h(\bx_t^{(0)} \cdot \hat{\bbeta}_{m}^{(0)})$ and collect data $(\hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})$.
}

\KwOutput{Offered price $\hat{p}_t^{(0)}$, $t \geq 1$}
\end{algorithm}



\begin{algorithm}[!ht]
\caption{Online-to-online Cross-Market Pricing Transfer in RKHS} \label{algo:trans-pricing-single-o2o-rkhs}
\KwInput{Online source market data $\{(\bp_t^{(k)}, \bX_t^{(k)}, \by_t^{(k)})\}_{t \in \calH^{(k)}}$ for $k \in [K]$; feature matrix $\{\bX_t^{(0)}\}_{t \in \mathbb{N}}$ for the target market}

Initialize: $l_1 \leftarrow 1$, $p_1^{(0)} \leftarrow 0$, $\hat{g}_0^{(0)} \leftarrow 0$ (zero function in $\mathcal{H}$)

\tcc{******* Aggregate and Debias *******}
\For{each episode $m = 2, 3,\ldots$} {
    \begin{align*}
         \hat{g}^{\rm (ag)}_m &= \argmin_{g \in \mathcal{H}_1} \Bigg\{ \frac{1}{Kl_{m-1}} \sum_{k \in [K]} \sum_{t \in \calH^{(k)}_{m-1}} L(g; p_t^{(k)}, \bx_t^{(k)}, y_t^{(k)}) + \lambda_{ag} \|g\|_{\mathcal{H}}^2 \Bigg\},\\
         \hat{\delta}_m &= \argmin_{\delta \in \mathcal{H}_2} \Bigg\{ \frac{1}{\ell_{m-1}} \sum_{t=2^{m-2}}^{2^{m-1}-1} L(\hat{g}^{\rm (ag)}_m + \delta; \hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)}) + \lambda_{tf} \|\delta\|_{\mathcal{H}}^2 \Bigg\},
    \end{align*}

    and set
    \begin{equation*}
        \hat{g}_m^{(0)} := \hat{g}^{\rm (ag)}_m + \hat{\delta}_m.
    \end{equation*}
    
    Apply price $\hat{p}_t^{(0)} :=  h(\hat{g}_m^{(0)}(\bx_t^{(0)}))$, and collect new data $(\hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})$.
}

\KwOutput{Offered price $\hat{p}_t^{(0)}$, $t \geq 1$}
\end{algorithm}


\begin{algorithm}[!ht]
\caption{Offline-to-online Cross-Market Pricing Transfer in RKHS} \label{algo:trans-pricing-single-f2o-rkhs}
\KwInput{Offline source market data $\{(\bp_t^{(k)}, \bX_t^{(k)}, \by_t^{(k)})\}_{t \in \calH^{(k)}_m}$ for $k \in [K]$; feature matrix $\{\bX_t^{(0)}\}_{t \in \mathbb{N}}$ for the target market}

\tcc{******* Initial Warm-up *******}
Compute the initial aggregated estimator $\hat{g}^{\rm (ag)}$ via Kernel Logistic Regression (KLR):
    \begin{equation*}
        \hat{g}^{\rm (ag)} = \argmin_{h \in \mathcal{H}_1} \Bigg\{ \frac{1}{n_\calK} \sum_{k \in [K]} \sum_{t \in \calH^{(k)}_{m-1}} L(g; p_t^{(k)}, \bx_t^{(k)}, y_t^{(k)}) + \lambda_{ag} \|g\|_{\mathcal{H}}^2 \Bigg\}.
    \end{equation*}

Apply price  $\hat{p}_1^{(0)}  := h(\hat{g}^{(ag)}(\bx_t^{(0)}))$ and collect data $(\hat{p}_1^{(0)}, \bx_1^{(0)}, y_1^{(0)})$.


\tcc{******* Update Estimate with transfer learning *******}
\For{each episode $m = 2, 3,\ldots, m_0$} {

    \begin{equation*}
        \hat{\delta}_m = \argmin_{\delta \in \mathcal{H}_2} \Bigg\{ \frac{1}{\ell_{m-1}} \sum_{t=2^{m-2}}^{2^{m-1}-1} L(\hat{g}^{\rm (ag)} + \delta; \hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)}) + \lambda_{tf} \|\delta\|_{\mathcal{H}}^2 \Bigg\},
    \end{equation*}
    and set
    \begin{equation*}
        \hat{g}_m^{(0)} := \hat{g}^{\rm (ag)}_m + \hat{\delta}_m.
    \end{equation*}
    Apply price $\hat{p}_t^{(0)} :=  h(\hat{g}_m^{(0)}(\bx_t^{(0)}))$, and collect new data $(\hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})$.
}

\tcc{******* Update Estimate without transfer learning *******}

\For{each $m \geq m_0 + 1$} {

\begin{equation*}
        \hat{g}^{(0)}_m = \argmin_{h \in \mathcal{H}_1} \Bigg\{ \frac{1}{\ell_{m-1}} \sum_{t=2^{m-2}}^{2^{m-1}-1} L(g; p_t^{(k)}, \bx_t^{(k)}, y_t^{(k)}) + \lambda \|g\|_{\mathcal{H}}^2 \Bigg\}.
\end{equation*}

Apply price $\hat{p}_t^{(0)} :=  h(\hat{g}_m^{(0)}(\bx_t^{(0)}))$, and collect new data $(\hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})$.

}

\KwOutput{Offered price $\hat{p}_t^{(0)}$, $t \geq 1$}
\end{algorithm}

==> NeurIPS2025/8-extension.tex <==
The proposed transfer pricing framework exhibits significant modularity and extensibility. Its core architecture—comprising source market aggregation and target-specific bias correction—can be seamlessly integrated with various existing pricing algorithms. This approach proves particularly valuable in scenarios characterized by limited historical data or evolving market conditions, subject to two fundamental conditions:

\begin{enumerate}
    \item The demand model must support parameter transferability, as is the case with linear models, logistic models, and other generalized linear model specifications.
    \item Market heterogeneity must be expressible through sparse parameter deviations between source and target markets.
\end{enumerate}

\subsection{Logistic Bandit Framework}
The logistic bandit formulation emerges as a natural extension, particularly suited for binary sales observations. In this setting, the purchase probability follows:

\[
\mathbb{P}(y_t^{(0)} = 1 | p_t, \bx_t^{(0)}) = \sigma\left(\langle \bx_t^{(0)}, \bbeta^{(0)} \rangle - \alpha p_t\right),
\]

where $\sigma(\cdot)$ denotes the logistic function and $\alpha$ represents price sensitivity. The optimal policy navigates the exploration-exploitation tradeoff by simultaneously learning $\bbeta^{(0)}$ while maximizing immediate revenue.

We validate this approach through simulations, detailed in Appendix \ref{app:general-exp}. Results again show that our transfer learning method achieves lower regret compared to learning from scratch, particularly when the target market has limited initial data. The improvement is most significant when the source and target markets share similar underlying demand structures.  

\subsection{Broader Applications}
The underlying transfer learning paradigm extends naturally to several advanced pricing scenarios:

\begin{itemize}
    \item \textbf{Bayesian Methods:} Thompson sampling variants that incorporate source-derived priors
    \item \textbf{Nonlinear Demand:} Neural network or kernel-based approaches with transfer initialization
    \item \textbf{Multi-product Settings:} Cross-category demand estimation in revenue management systems
\end{itemize}

These extensions maintain the core benefits of our approach while addressing more complex, real-world pricing challenges where data sparsity and market heterogeneity are prevalent. 

==> NeurIPS2025/9-check-list.tex <==
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction clearly outline the paper's key contributions, including the development of a novel transfer learning algorithm for dynamic pricing, theoretical analysis of the algorithm, and experimental validations. The claims are supported by the theoretical framework presented in Section \ref{sec:prob-setting} and the experimental results detailed in Section \ref{sec:exps}, aligning with the guidelines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:\answerYes{}
    \item[] Justification: Although not labeled under a "Limitations" section, limitations are implicitly discussed in the assumptions underlying the theoretical results, such as paramter space in in Assumption \ref{assump:param}, homogeneity in design matrices in Assumption \ref{assump:Homo-Cov}, known noise distributions, and sparsity constraints on parameters in Assumption \ref{assump:simi_sparsity-linear}. These limit generalizability and are explicitly stated.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper provide the full set of assumptions and a complete (and correct) proof for both online to online and offline to online transfer learning setting, with an outline for the proof following the statement of Theorem \ref{thm:upper-single-homo-linear-o2o} and \ref{thm:upper-single-homo-linear}, and complete versions in Appendix \ref{apd:upper-single-homo-linear-o2o} and \ref{apd:upper-single-homo-linear}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Although the paper is primarily theoretical, focusing on algorithm design, regret analysis, and proofs under well-defined assumptions, we still include empirical experiments accompanied with open soirce code and data for validation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: Our implementation is available at \url{https://github.com/CS-SAIL/transfer_pricing_neurips2025}, including a README with setup instructions, usage examples, and reproduction steps.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper specifies all the necessary experiment setup in Section \ref{sec:exps}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper reports confidence intervals in numerical experiments, as demonstrated in Figures~\ref{fig:regret-linear-on}, \ref{fig:regret-rkhs-on}, \ref{fig:regret-linear-off} and \ref{fig:regret-rkhs-off}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Information on the computer resources is specified in Appendix~\ref{apd:off2on}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The research conducted in the paper conform with the NeurIPS Code of Ethics in every respect.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper includes a discussion in Section \ref{sec:conclusion} that clearly outlines potential positive and negative societal impacts, such as improving pricing efficiency, supporting small businesses, and enhancing customer satisfaction through adaptive pricing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}
    \item[] Justification: All assets used in the paper, including code and models, are our own work. Therefore, no external creators or original owners need to be credited; licenses and terms of use for external assets are not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper mentions a new asset in the form of Python code, which is available at \url{ https://github.com/CS-SAIL/transfer_pricing_neurips2025}. Detailed user guide, API reference, and installation instructions are provided alongside the asset in the README.md file.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects. The paper appears to focus entirely on theoretical modeling, algorithm development, and regret analysis within simulated or synthetic environments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects. The paper appears to focus entirely on theoretical modeling, algorithm development, and regret analysis within simulated or synthetic environments. There is no mention of human subject experiments, surveys, or deployment in real-world platforms that would necessitate IRB review.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper doesn't use LLMs for any important, original, or non-standard component of the core methods in this research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> NeurIPS2025/old-introduction.tex <==
\section{Introduction}

In the era of data-driven decision-making, pricing strategies have become increasingly complex and dynamic. This paper introduces a novel approach to dynamic pricing, leveraging the power of transferred knowledge from related markets. We propose a Cross-Market Transfer Dynamic Pricing (MMCP-TDP) framework that combines machine learning and transfer learning techniques to optimize pricing strategies in real-time.

The Cross-TDP framework capitalizes on the availability of data from multiple markets, where pricing dynamics exhibit similarities. By transferring knowledge from these source markets to the target market, we enable more efficient pricing decisions, even in situations with limited historical data.

Key contributions of our research include the development of a transfer learning algorithm tailored for pricing, allowing for the adaptation of pricing models to changing market conditions. We demonstrate the effectiveness of our approach through extensive experiments on diverse datasets, highlighting improvements in pricing accuracy, revenue generation, and customer satisfaction.

Furthermore, we address the practical challenges of implementing MMCP-TDP in real-world scenarios, including data integration, model deployment, and scalability. Our findings reveal that MMCP-TDP not only enhances pricing performance but also provides valuable insights into market dynamics and customer behavior.

This research opens new horizons for businesses seeking to optimize their pricing strategies in dynamic environments. By harnessing the power of transferred knowledge, MMCP-TDP offers a promising avenue for companies to stay competitive and adapt to rapidly evolving market conditions.

{\blue
For any candidate function $g \in \mathcal{G}$, the transferability is quantified via:

\begin{enumerate}[leftmargin=1.45em,itemsep=1pt]
\item \emph{Parameter-based similarity:} When $\mathcal{G}$ is parametric, market relationships are encoded through constraints on the parameter deviations $\| \beta^{(k)} - \beta^{(0)} \|_{\mathcal{T}}$ where $\mathcal{T}$ is a problem-specific norm capturing the transfer structure.
\item \emph{Representation-based similarity:} For non-parametric $\mathcal{G}$, similarity is measured through the induced functional discrepancy $\sup_{x \in \mathcal{X}} |g^{(k)}(x) - g^{(0)}(x)|_{\mathcal{R}}$ where $\mathcal{R}$ is an appropriate function space metric.
\end{enumerate}


This unified characterization accommodates both linear and nonlinear utility models while maintaining the core transfer learning paradigm: source markets are considered informative when either their parameter deviations or functional differences are bounded within a recoverable neighborhood of the target market.
}

\begin{algorithm}[!ht]
\caption{CM-TDP-\textsc{O2O\textsubscript{on}}} \label{algo:general-o2o}
\KwInput{Streaming source data $\!\{(p_t^{(k)},\bx_t^{(k)},y_t^{(k)})\}_{t\ge1}\!$ for $k\in[K]$; \\
\hspace{6ex}streaming target contexts $\{\bx_t^{(0)}\}_{t\ge1}$}

\textbf{Initialization:} $\ell_1 \leftarrow 1$, $\cT_m = [1]$, $p_1^{(0)} \leftarrow 0$, $\hat{\mathring{g}}_0^{(0)} \leftarrow 0$

\tcc{******* Phased-based Doubling Scheduling *******}
\For{each episode $m = 2, 3,\ldots$} {Compute $\ell_m\!=\!2^{m-1}$, $\cT_m = [\ell_m, \ell_{m+1}-1]$. 

\tcc{******* Two–step \emph{bias-corrected aggregation} framework *******}
(Aggregation): Using source market data $\{(\bp_t^{(k)}, \bX_t^{(k)}, \by_t^{(k)})\}_{t \in \cT_{m-1}}$ for $k \in [K]$, call \texttt{Algorithm \ref{algo:mle} for linear utility} (or \texttt{Algorithm \ref{algo:krr} for non-parametric utility}) to calculate the aggregated estimate $\hat{\mathring{g}}_m^{\rm (ag)}$. 

(Bias-correction): Using target market data $\{(p_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})\}_{t \in \cT_{m-1}}$ and aggregated estimate $\hat{\mathring{g}}^{\rm (ag)}$, call \texttt{Algorithm \ref{algo:mle} for linear utility} (or \texttt{Algorithm \ref{algo:krr} for non-parametric utility}) to calculate the debiasing estimate $\hat{\delta}_m$.

Set
\begin{equation*}
    \hat{\mathring{g}}_m^{(0)} := \hat{\mathring{g}}_m^{\rm (ag)} + \hat{\delta}_m.
\end{equation*}

\For{each time $t \in \cT_m$} {
\tcc{******* Greedy Pricing for Episode $m$ *******}
Set price $\hat{p}_t^{(0)} := h(\hat{\mathring{g}}_{m}^{(0)}(\bx^{(0)}_t))$ and collect data $(\hat{p}_t^{(0)}, \bx_t^{(0)}, y_t^{(0)})$.
}
}
\KwOutput{Offered price $\hat{p}_t^{(0)}$, $t \geq 1$}
\end{algorithm}

==> literature.tex <==


Transfer learning has been actively studied recently, with applications in areas such as recommendation systems (e.g. Pan et al., 2010), language models (e.g. Han et al., 2021) and disease detection (e.g. Maqsood et al., 2019). 
It has recently also gained attention in statistics and has been explored in various problems, such as
nonparametric regression (Cai and Pu, 2022), contextual multi-armed bandits (Suk and Kpotufe,
2021; Cai et al., 2024a) and functional data analysis (Cai et al., 2024b). In statistical transfer
learning, two common settings are posterior drift, where the conditional distributions of responses
given covariates vary (e.g. Maity et al., 2022; Reeve et al., 2021), and covariate shift, where the
conditional distributions remain consistent but the marginal distributions of covariates differ (e.g.
Hanneke and Kpotufe, 2019; Kpotufe and Martinet, 2021).

Bastani \cite{bastani2021predicting} studies the transfer learning problem of high-dimensional linear regression and proposes a two-step estimator, which efficiently combines the source and target data and provides the upper bound of the estimation error. 

\cite{tullii2024improved} present VAPE, a unified exploration–exploitation algorithm that uses random pricing and cross-context information pooling to achieve minimax-optimal $T^{2/3}$ regret for linear and near-optimal rates for H\'{o}lder non-parametric contextual dynamic pricing under minimal Lipschitz-noise assumptions.

Huang et al.\cite{huang2025optimal} proposes a weighted-median-based multitask estimator (MOLAR) and its bandit analogue that exploit sparse heterogeneity across tasks to achieve minimax-optimal error rates and regret in linear regression and contextual bandits.

\smallskip
\noindent
\textbf{Multi-Task and Transfer Learning for Dynamic Pricing.} 
Bastani et al. \cite{bastani2022meta} introduce meta-learning variants of Thompson sampling that estimate a shared Gaussian prior across multiple products. 
Bastani, Simchi-Levi, and Zhu’s “Meta Dynamic Pricing” learns a shared Bayesian prior across \emph{sequential} product experiments and speeds Thompson-sampling pricing via meta-exploration, whereas our method transfers \emph{concurrently} across markets under utility-parameter shift and is analysed with frequentist regret bounds.
\cite{wang2025transfer} introduces a covariate-shift-aware transfer-learning scheme that warm-starts contextual zooming with source-market data, yielding minimax-optimal regret for nonparametric contextual dynamic pricing and continuously tighter bounds as source-target similarity and sample size increase. 


\section{Related Work}

\section{Related Work}\label{sec:related}

\noindent
\textbf{Contextual Dynamic Pricing in a Single Market (no transfer).}  
Pioneering studies assumed that a product’s valuation is a \emph{deterministic} function of observable covariates, most commonly linear, yielding algorithms with sub-linear regret in that setting~\cite{amin2014repeated,cohen2020feature,liu2021optimal}.  A few works relaxed linearity and analysed non-parametric (kernel- or tree-based) valuations instead~\cite{mao2018contextual}.  

More recent research embraces \emph{random} valuations: the consumer’s latent value equals a covariate-dependent mean utility plus i.i.d.\ noise.  With a \emph{known} noise distribution, \cite{javanmard2019dynamic} derived the first regret bounds for linear utilities.  Follow-up papers removed the knowledge-of-noise assumption but retained linearity, proposing doubly robust or moment-matching estimators to handle the unknown noise~\cite{xu2022towards,luo2022contextual,fan2024policy}.  \cite{tullii2024improved} tightened these bounds to the information-theoretic optimum for linear utilities and extended the analysis to H\"older-smooth (non-parametric) demand curves, while \cite{chen2024dynamic} studied a fully non-parametric utility under unknown noise.

All of the above methods must \emph{learn from scratch} in every new market and therefore deteriorate when the target data set is small.  In contrast, we consider \emph{multiple} markets whose mean utilities differ by a structured \emph{utility shift}.  The proposed MMCP-TDP exploits this similarity to accelerate learning for \emph{both} sparse-linear and RKHS-smooth utilities.  To the best of our knowledge, our RKHS analysis yields the first regret guarantees for dynamic pricing with kernel-based (non-parametric) valuations.

\smallskip
\noindent
\textbf{Transfer and Meta-Learning for Dynamic Pricing.}
The idea of exploiting cross-product transfer first appeared in the \emph{meta dynamic pricing} framework \citep{bastani2022meta}. They consider the linear demand function where the demands are directly observable and introduce meta-learning variants of Thompson sampling that estimate a shared Gaussian prior across multiple products. In contrast, we employ the random utility model where the demand is a non-linear function of contextual information or price. 
Recently, \citep{wang2025transfer} introduced TLDP, a \emph{non-parametric} transfer-learning algorithm for contextual pricing under \emph{covariate shift}, together with matching minimax bounds—but only for an \emph{offline-to-online, one-source} setting. 
Our CM-TDP framework is the first transfer dynamic pricing framework considers the \emph{utility model shift}. 
In addition, we generalize this line by (i) allowing \emph{multiple} simultaneous sources, (ii) handling both linear and RKHS utilities, and  (iii) delivering sharper $\tilde{\mathcal O}\!\bigl((d/K+s_0)\log T\bigr)$ or $T^{(\eta+1)/(2\eta+1)}$ regret in fully online operation.

\smallskip
\noindent
\textbf{Multitask \& Transfer Learning in Contextual Bandits.} Beyond pricing, multitask estimators for linear contextual bandits provide transferable confidence sets that shrink with cross-task similarity. 
\cite{cai2024transfer} tackles the covariate-(domain-)shift case - source and target share the same reward model while the feature distribution changes - proving minimax-optimal regret bounds, whereas our work allow the reward parameters themselves to change across tasks. 
Xu et al. \cite{xu2025multitask} introduce a robust two-stage multitask estimator that leverages trimmed-mean aggregation and LASSO debiasing to exploit sparse heterogeneity. MOLAR \cite{huang2025optimal} employs a weighted-median / debiasing scheme to obtain minimax-optimal regret under \emph{sparse heterogeneity}.   
Complementary work tackles negative transfer via causal transportability in latent contextual bandits, showing that naive pooling can be provably harmful under covariate shift \citep{deng2025transfer}.   
\cite{chen2022transfer,chen2024data,chai2025deep, chai2025transition} considers reward and transition transfers for reinforcement learning. 
Our bias-correction step is inspired by these robust multitask estimators but is tailored to revenue objectives and pricing-specific structure.

\smallskip
\noindent
\textbf{Online Meta-Learning Without Task Boundaries.} Fully online meta-learning algorithms such as FOML \citep{rajasegaran2022fully} and Online-within-Online meta-learning \citep{denevi2019online} adapt to continuously drifting task distributions without explicit task resets. 
MMCP-TDP shares the same spirit - episodes are used only for analysis; the algorithm itself runs in a single stream - yet differs in that it must optimize \emph{actions} (prices) rather than predictions, and thus balances exploration - exploitation through regret-aware pricing rules.

\smallskip
\noindent
\textbf{Positioning of This Work.} To our knowledge, ours is the first dynamic-pricing method that
\emph{(i)} simultaneously leverages multiple auxiliary markets (online or offline),
\emph{(ii)} provides provably optimal regret bounds for both sparse‐linear and RKHS utilities, and
\emph{(iii)} unifies bias-corrected aggregation with revenue-maximising price selection.
This bridges the gap between single-market pricing algorithms \citep{tullii2024improved}, meta-learning approaches that learn priors offline \citep{bastani2022meta,chen2025distributed}, and multitask bandit estimators such as MOLAR that focus on prediction error rather than economic objectives.

\section{Shorter Version}

\section{Related Work}\label{sec:related}

\noindent
\textbf{Single-market contextual pricing.}
Classical algorithms assume a \emph{deterministic} valuation map-usually linear-and attain sub-linear regret~\cite{amin2014repeated,cohen2020feature,liu2021optimal}; non-parametric variants are analyzed in~\cite{mao2018contextual}.  
The current benchmark is the \emph{random-utility} model: linear mean plus i.i.d.\ noise.  
With known noise, \cite{javanmard2019dynamic} give the first bounds; unknown-noise counterparts use doubly robust or moment matching estimators~\cite{xu2022towards,luo2022contextual,fan2024policy}.  
\cite{tullii2024improved} close the gap to the information-theoretic optimum for linear utilities and extend to H\"older-smooth demand, while \cite{chen2024dynamic} provide fully non-parametric guarantees.  
All of these methods restart learning in every market, hurting performance when the target data set is small.

\noindent
\textbf{Transfer and meta learning for pricing.}
\emph{Meta Dynamic Pricing} pools directly observed linear demands and learns a shared Gaussian prior across products~\cite{bastani2022meta}.  
TLDP transfers under pure \emph{covariate(domain) shift} but only from one offline source~\cite{wang2025transfer}.  
Our CM-TDP differs by handling \emph{utility-model} shift, supporting multiple online/offline sources, and covering both sparse-linear and RKHS utilities.

\noindent
\textbf{Multitask contextual bandits and RL.}
Domain-shift transfer for bandits is studied in~\cite{cai2024transfer}; sparse heterogeneity is tackled via trimmed-mean and LASSO debiasing~\cite{xu2025multitask} or weighted-median MOLAR~\cite{huang2025optimal}.  
Causal-transport ideas expose negative transfer risks~\cite{deng2025transfer}.  
Reward/transition transfer in RL is addressed by~\cite{chen2022transfer,chen2024data,chai2025deep,chai2025transition}.  
We adapt these bias-correction techniques to revenue maximisation under shifting utilities.

\noindent
\textbf{Fully online meta learning.}
FOML~\cite{rajasegaran2022fully} and online-within-online updates~\cite{denevi2019online} learn without explicit task boundaries.  
CM-TDP inherits this streaming design but must manage exploration-exploitation through posted prices rather than prediction loss.

\noindent
\textbf{Positioning of This Work.}
Our contribution is the first dynamic-pricing framework that 
\emph{(i)} transfers across \emph{multiple} markets under \emph{utility model shift}, 
\emph{(ii)} achieves minimax-type regret for both linear and RKHS utilities, and 
\emph{(iii)} unifies bias-corrected aggregation with revenue-maximising pricing, thereby connecting single-market pricing~\cite{tullii2024improved}, offline meta-priors~\cite{bastani2022meta,chen2025distributed}, and multitask bandits~\cite{huang2025optimal}.
